Wakening Past Concepts without Past Data: Class-Incremental Learning from Online Placebos

Not forgetting old class knowledge is a key challenge for class-incremental learning (CIL) when the model continuously adapts to new classes. A common technique to address this is knowledge distillation (KD), which penalizes prediction inconsistencies between old and new models. Such prediction is made with almost new class data, as old class data is extremely scarce due to the strict memory limitation in CIL. In this paper, we take a deep dive into KD losses and find that "using new class data for KD" not only hinders the model adaption (for learning new classes) but also results in low efficiency for preserving old class knowledge. We address this by "using the placebos of old classes for KD", where the placebos are chosen from a free image stream, such as Google Images, in an automatical and economical fashion. To this end, we train an online placebo selection policy to quickly evaluate the quality of streaming images (good or bad placebos) and use only good ones for one-time feed-forward computation of KD. We formulate the policy training process as an online Markov Decision Process (MDP), and introduce an online learning algorithm to solve this MDP problem without causing much computation costs. In experiments, we show that our method 1) is surprisingly effective even when there is no class overlap between placebos and original old class data, 2) does not require any additional supervision or memory budget, and 3) significantly outperforms a number of top-performing CIL methods, in particular when using lower memory budgets for old class exemplars, e.g., five exemplars per class.

==> figures/acc.tex <==
\begin{figure*}[ht]
\newcommand{\newincludegraphics}[1]{\includegraphics[height=1.26in]{#1}}
\centering
\includegraphics[height=0.2in]{files/legend.pdf}
%\vspace{0.21cm}
\subfigure[CIFAR-100 ($100$ classes).]{
\newincludegraphics{files/cifar100_5phase.pdf}

\hspace{-1mm}
\newincludegraphics{files/cifar100_10phase.pdf}
\hspace{-1mm}
\newincludegraphics{files/cifar100_25phase.pdf}
}

\subfigure[ImageNet-100 ($100$ classes).]{
\newincludegraphics{files/imagenetsub_5phase.pdf}

\hspace{-1mm}
\newincludegraphics{files/imagenetsub_10phase.pdf}
\hspace{-1mm}
\newincludegraphics{files/imagenetsub_25phase.pdf}
}




\vspace{0.2cm}
\caption{\suppt{Supplementary to Table~2.} Phase-wise accuracies ($\%$) on CIFAR-100 and ImageNet-100. 
}
\label{figure_acc_plots}
\cotronlvsapce
\end{figure*}



==> figures/global_flow.tex <==
\begin{figure*}[t]

\includegraphics[width=\textwidth]{files/global-flow.pdf}
\vspace{-0.6cm}
\caption{The computing flow of our method. We formulate the CIL task as an online MDP: each phase in CIL is a stage in the MDP, and the CIL models are the states. We train the policy to produce actions, which contain the hyperparameters we use in the CIL training. We illustrate the training process of each phase in Figure~xxx.}
\vspace{-0.4cm}
  \label{global_figure}
\end{figure*}

==> tables/ablation_2.tex <==
\begin{wraptable}{r}{8.7cm}
\vspace{-1mm}
	\begin{minipage}{0.64\textwidth}
		\begin{minipage}[t]{\textwidth}
			\vspace{7pt}
			\centering
			\resizebox{\textwidth}{!}{
%\begin{table*}%[ht]
  \small
  \centering
  \begin{tabular}{llccccccccccc}
  \toprule
      %\\[-11pt]
    \multirow{2.5}{*}{No.}&\multirow{2.5}{*}{Setting} & \multicolumn{2}{c}{LwF} && \multicolumn{2}{c}{iCaRL}\\
        %\\[-11pt]
  \cmidrule{3-4} \cmidrule{6-7} 
      %\\[-11pt]
   && Average & Last  && Average & Last \\
       %\\[-11pt]
    \midrule
        %\\[-11pt]
    1&Baseline & 53.19   & 43.18  && 57.12   & 47.49  && 63.17  & 53.71 && 66.72   & 57.77 \\
          %\\[-11pt]
    2&PlaceboCIL (budget)  & 59.10 & 48.28 && 61.09 & 50.81 && 65.14 & 56.95 && 67.31 & 59.26\\
          %\\[-11pt]
    3&PlaceboCIL (non-budget) & 59.29   & 49.64  && 61.17   & 50.96 && 65.48  & 56.77  && 67.33  & 59.32 \\
        %\\[-11pt]
    \midrule
        %\\[-11pt]
    4&Overlapping & 58.95   & 48.71  && 62.15   & 52.62 && 65.73  & 57.26  && 67.48  & 59.06 \\
          %\\[-11pt]
    5&Non-overlapping & 58.59   & 49.28  && 61.52   & 51.70  && 65.48  & 56.99 && 67.01  & 58.53 \\
          %\\[-11pt]
    6&New data & 54.06   & 43.94  && 57.70  & 47.51  && 64.21  & 53.98 && 66.69 & 57.33 \\
          %\\[-11pt]
    7&Old data (upper bound)& 61.41  & 51.16 && 66.64 & 58.03 && 67.02 & 58.98 && 68.82 & 61.52 \\
        %\\[-11pt]
    \midrule
        %\\[-11pt]
    8&\emph{w/o} RL  & 57.06  & 46.12  && 60.27 & 50.57  && 63.83 & 55.33 && 66.91 & 58.88 \\
          %\\[-11pt]
    9&\emph{w/} Transferred RL  & 58.36  & 48.98 && 61.58  & 52.51  && 65.04  & 56.48 &&  67.18 & 57.84\\
        %\\[-11pt]
    \midrule
        %\\[-11pt]
    10&CE loss on placebos  & 56.23  & 45.74 && 56.40  & 44.70 && 65.03 & 55.84 && 66.05 & 56.02 \\
    \midrule
        %\\[-11pt]
    \revision{11}&\revision{Higher confidence} &\revision{56.98}&\revision{46.20}&&\revision{60.43}&\revision{49.36} && \revision{63.60}&\revision{55.50} && \revision{--} & \revision{--} \\
    \revision{12}&\revision{Random placebos} &\revision{50.99}&\revision{40.22}&&\revision{56.27}&\revision{46.64} && \revision{64.16}&\revision{55.450} && \revision{66.23} & \revision{57.22} \\
    %\\[-11pt]
    
    
  \bottomrule

\end{tabular}
	%}
		%\end{minipage}
		\centering
  \vspace{-0.2cm}
	\caption{Ablation results (\%) on CIFAR-100, $N$=$5$.``Average'' and ``Last'' denote the average accuracy over all phases and the last-phase accuracy, respectively. The four blocks show the results of baselines, using different free image streams, using RL (or not), and using placebos to compute CE loss, respectively. Please refer to more details in Section~\ref{subsec_exp_analyses} \textbf{Ablation study}.}
	\label{table_ablation_2}	
  \vspace{-0.2cm}
%\end{table*}
	\end{minipage}
	\end{minipage}
\end{wraptable}

==> tables/ablation_mem.tex <==

\begin{table*}[ht]
  \small
  \centering
   \setlength{\tabcolsep}{1.05mm}{
  \begin{tabular}{llccccccccccc}
  \toprule
      \\[-11pt]
    \multirow{2.5}{*}{No.}&\multirow{2.5}{*}{Setting} & \multicolumn{2}{c}{LwF} && \multicolumn{2}{c}{iCaRL} && \multicolumn{2}{c}{LUCIR} && \multicolumn{2}{c}{AANets}\\
        \\[-11pt]
  \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}
      \\[-11pt]
   && Average & Last  && Average & Last && Average & Last && Average & Last\\
       \\[-11pt]
    \midrule
        \\[-11pt]
    1&Baseline & 53.19   & 43.18  && 57.12   & 47.49  && 63.17  & 53.71 && 66.72   & 57.77 \\
          \\[-11pt]
    2&PlaceboCIL (budget)  & 59.06 & 48.56 && 61.01 & 51.45 && 65.42 & 56.18 && 67.16 & 59.14\\
          \\[-11pt]
    3&PlaceboCIL (non-budget) & 59.08  & 49.15  && 61.24 & 51.47 && 65.28 & 56.23 && 67.27  & 59.15\\
        \\[-11pt]

    
    
  \bottomrule

\end{tabular}
}
	%}
		%\end{minipage}
		\centering
  \vspace{-0.2cm}
	\caption{
	Ablation results (\%) on CIFAR-100, $N$=$5$.``Average'' and ``Last'' denote the average accuracy over all phases and the last-phase accuracy, respectively.}
	\vspace{-0.3cm}
	\label{table_ablation_mem}
\end{table*}

==> tables/ablation_more.tex <==
\setlength{\tabcolsep}{3.2mm}{
\begin{table*}[ht]
\centering
  \vspace{-0.0cm}
 \begin{tabular}{llccccccccccc}
  \toprule
      \\[-11pt]
    \multirow{2.5}{*}{No.}&\multirow{2.5}{*}{Setting} & \multicolumn{2}{c}{LwF} && \multicolumn{2}{c}{LUCIR} \\
        \\[-11pt]
  \cmidrule{3-4} \cmidrule{6-7} 
      \\[-11pt]
   && Average & Last  && Average & Last \\
         \\[-11pt]
    \midrule
        \\[-11pt]
    1&Baseline & 53.19   & 43.18  && 63.17  & 53.71  \\
          \\[-11pt]
    2&PlaceboCIL  & 59.06 & 48.56 && 65.42 & 56.18\\
          \\[-11pt]
        \\[-11pt]
    \midrule
        \\[-11pt]
    3&Overlapping & 58.95   & 48.71  && 65.73  & 57.26 \\
          \\[-11pt]
    4&Non-overlapping & 58.59   & 49.28  && 65.48  & 56.99 \\
          \\[-11pt]
    5&New data & 54.06   & 43.94  && 64.21  & 53.98 \\
          \\[-11pt]
    6&Old data (oracle)& 61.41  & 51.16 && 67.02 & 58.98 \\
        \\[-11pt]
    \midrule
        \\[-11pt]
    7&\emph{w/o} Online learning  & 57.06  & 46.12  && 63.83 & 55.33  \\
          \\[-11pt]
    8&Offline RL& 59.01   & 48.18  && 65.14  & 56.95  \\
        \\[-11pt]
    \midrule
        \\[-11pt]
    \revision{9}&\revision{Higher confidence} &\revision{56.98}&\revision{46.20}&&\revision{63.60}&\revision{55.50}  \\
    \revision{10}&\revision{Random placebos} &\revision{50.99}&\revision{40.22}&&\revision{64.16}&\revision{55.40}  \\
    \\[-11pt]
    
    
  \bottomrule
\end{tabular}
  	\centering
	\caption{Ablation results (\%) on CIFAR-100, $N$=$5$.}
	\label{table_ablation_more}
 \vspace{-0.4cm}
\end{table*}
}

==> tables/equal.tex <==
\setlength{\tabcolsep}{1.7mm}{
\begin{table*}[ht]
  \small
  \centering
  \begin{tabular}{llccccccccccc}
  \toprule
      \\[-11pt]
    \multirow{2.5}{*}{No.}&\multirow{2.5}{*}{Setting} & \multicolumn{2}{c}{LwF} && \multicolumn{2}{c}{iCaRL} && \multicolumn{2}{c}{LUCIR} \\
        \\[-11pt]
  \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} 
      \\[-11pt]
   && Average & Last  && Average & Last && Average & Last \\
       \\[-11pt]
    \midrule
        \\[-11pt]
    1&   Baseline &53.85&41.00&&59.70&45.29&&56.71&42.78\\
  2&PlaceboCIL (ours) &57.68&42.44&&62.32&46.52&&57.89&44.08\\
  3&PlaceboCIL (ours, w/o online learning) &56.31&41.76&&61.05&46.02&&57.01&43.13\\
    
  \bottomrule

\end{tabular}
	%}
		%\end{minipage}
		\centering
  \vspace{-0.2cm}
	\caption{\suppt{Supplementary to Table~\ref{table_ablation_2}.}
  Ablation results (\%) using equal-size split on CIFAR-100, $10$-phase ($10$ classes/phase). }
	\label{table_ablation_equal}
 \vspace{-0.5cm}
\end{table*}
}

==> tables/lca.tex <==
\setlength{\tabcolsep}{2mm}{
\begin{table}[htp]
  \small
  \centering
  \begin{tabular}{llcccccccc}
  \toprule
   \multirow{2}{*}{No.}&\multirow{2}{*}{Setting} &  \multirow{2}{*}{LwF} &  \multirow{2}{*}{iCaRL} & \multirow{2}{*}{LUCIR} & LUCIR\\
   &&&&&+AANets\\
   \midrule
   1&Baseline &40.02&47.79&52.06&56.44\\
  2& PlaceboCIL (ours) &50.82&55.24&57.48&59.69\\
  \bottomrule
\end{tabular}
\caption{\suppt{Supplementary to Table~\ref{table_ablation_2}.}
  Learning Curve Area (LCA$_{10}$)~\citep{chaudhry2018efficient} on CIFAR-100, $5$-phase. }
  \label{table_lca}
\end{table}
}

==> tables/new_ablation_backup.tex <==
\begin{wraptable}{r}{7.6cm}
%\begin{table*}%[ht]
  \small
  \centering
  \setlength{\tabcolsep}{0.70mm}{
  \vspace{-0.0cm}
 \begin{tabular}{llccccccccccc}
  \toprule
      \\[-11pt]
    \multirow{2.5}{*}{No.}&\multirow{2.5}{*}{Setting} & \multicolumn{2}{c}{LwF} && \multicolumn{2}{c}{iCaRL} \\
        \\[-11pt]
  \cmidrule{3-4} \cmidrule{6-7} 
      \\[-11pt]
   && Average & Last  && Average & Last \\
       \\[-11pt]
    \midrule
        \\[-11pt]
    1&Baseline & 53.19   & 43.18  && 57.12   & 47.49  \\
          \\[-11pt]
    2&PlaceboCIL  & 59.06 & 48.56 && 61.01 & 51.45 \\
          \\[-11pt]
    \midrule
        \\[-11pt]
    3&Overlapping & 58.95   & 48.71  && 62.15   & 52.62  \\
          \\[-11pt]
    4&Non-overlapping & 58.59   & 49.28  && 61.52   & 51.70  \\
          \\[-11pt]
    5&New data & 54.06   & 43.94  && 57.70  & 47.51  \\
          \\[-11pt]
    6&Old data (oracle)& 61.41  & 51.16 && 66.64 & 58.03 \\
        \\[-11pt]
    \midrule
        \\[-11pt]
    7&\emph{w/o} Online learning  & 57.06  & 46.12  && 60.27 & 50.57  \\
          \\[-11pt]
    8&Offline RL& 59.01   & 48.18  && 61.09   & 50.81  \\
        \\[-11pt]
    \midrule
        \\[-11pt]
    \revision{9}&\revision{Higher confidence} &\revision{56.98}&\revision{46.20}&&\revision{60.43}&\revision{49.36}  \\
    \revision{10}&\revision{Random placebos} &\revision{50.99}&\revision{40.22}&&\revision{56.27}&\revision{46.64}  \\
    \\[-11pt]
    
    
  \bottomrule

\end{tabular}
}
	%}
		%\end{minipage}
		\centering
  \vspace{-0.3cm}
	\caption{Ablation results (\%) on CIFAR-100, $N$=$5$.
 }
	\label{table_ablation_2}
   \vspace{-0.2cm}

\end{wraptable}

==> tables/sources.tex <==
%\begin{wraptable}{r}{8.7cm}
%\vspace{-1mm}
%	\begin{minipage}{0.64\textwidth}
%		\begin{minipage}[t]{\textwidth}
%			\vspace{7pt}
%			\centering
%			\resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{0.90mm}{
\begin{table*}[ht]
  \small
  \centering
  \begin{tabular}{llccccccccccc}
  \toprule
      \\[-11pt]
    \multirow{2.5}{*}{No.}&\multirow{2.5}{*}{Setting} & \multicolumn{2}{c}{LwF} && \multicolumn{2}{c}{iCaRL} && \multicolumn{2}{c}{LUCIR} && \multicolumn{2}{c}{AANets}\\
        \\[-11pt]
  \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}
      \\[-11pt]
   && Average & Last  && Average & Last && Average & Last && Average & Last\\
       \\[-11pt]
    \midrule
        \\[-11pt]
    1&Baseline & 53.19   & 43.18  && 57.12   & 47.49  && 63.17  & 53.71 && 66.72   & 57.77 \\
          \\[-11pt]
          \\[-11pt]
    2&PlaceboCIL (ours, all) & 59.29   & 49.64  && 61.17   & 50.96 && 65.48  & 56.77  && 67.33  & 59.32 \\
        \\[-11pt]
    3&PlaceboCIL (ours, overlapping) & 58.95   & 48.71  && 62.15   & 52.62 && 65.73  & 57.26  && 67.48  & 59.06 \\
        \\[-11pt]
    4&{Random unlabeled data (all)} &{50.99}&{40.22}&&{56.27}&{46.64} && {64.16}&{55.45} && {66.23} & {57.22} \\
    \\[-11pt]
    4&{Random unlabeled data (overlapping)} &{50.80}&{40.94}&&{55.70}&{46.47} && {64.23}&{54.68} && {66.58} & {57.08} \\    
    \\[-11pt]   
  \bottomrule

\end{tabular}
	%}
		%\end{minipage}
		\centering
	\caption{\suppt{Supplementary to Table~\ref{table_ablation_2}.} Ablation results (\%) on CIFAR-100, $N$=$5$.``Average'' and ``Last'' denote the average accuracy over all phases and the last-phase accuracy, respectively. ``All'' denotes using all data from ImageNet, and ``overlapping'' means including samples from the overlapping classes between CIFAR-100 and ImageNet.}
	\label{table_ablation_source}	
\end{table*}}
%	\end{minipage}
%\end{wraptable}

==> tables/table_rebuttal.tex <==
\begin{table*}[ht]
  \small
  \centering
  \setlength{\tabcolsep}{0.70mm}{
 \begin{tabular}{llccccccccccc}
  \toprule
      %\\[-11pt]
      %\\[-11pt]
   {No.}&{Setting}  & Average & Last \\
       %\\[-11pt]
    \midrule
        %\\[-11pt]
    1&Baseline &  66.72  & 57.77  \\
          %\\[-11pt]
    2&PlaceboCIL (original) &  67.16 & 59.14 \\
    {3}&PlaceboCIL ({higher confidence}) &{66.97}&{58.12}  \\
    \midrule
    4&Baseline \emph{w/o} exemplars  &  50.01  & 39.12  \\
          %\\[-11pt]
    5&PlaceboCIL (original) \emph{w/o} exemplars  &  56.31 & 44.02 \\
    {6}&PlaceboCIL ({higher confidence}) \emph{w/o} exemplars &{53.41}&{41.93}  \\

    
  \bottomrule

\end{tabular}
}
	%}
		%\end{minipage}
		\centering
	\caption{Ablation results (\%) on CIFAR-100, $N$=$5$. Baseline: LUCIR+AANets~\cite{Liu2020AANets}.
 }
	\label{table_ablation_rebuttal_1}
   \vspace{0.0cm}

\end{table*}

